Controlling the Spread of Epidemics on Networks with Differential Privacy

Designing effective strategies for controlling epidemic spread by vaccination is an important question in epidemiology, especially in the early stages when vaccines are limited. This is a challenging question when the contact network is very heterogeneous, and strategies based on controlling network properties, such as the degree and spectral radius, have been shown to be effective. Implementation of such strategies requires detailed information on the contact structure, which might be sensitive in many applications. Our focus here is on choosing effective vaccination strategies when the edges are sensitive and differential privacy guarantees are needed. Our main contributions are $(\varepsilon,\delta)$-differentially private algorithms for designing vaccination strategies by reducing the maximum degree and spectral radius. Our key technique is a private algorithm for the multi-set multi-cover problem, which we use for controlling network properties. We evaluate privacy-utility tradeoffs of our algorithms on multiple synthetic and real-world networks, and show their effectiveness.

==> 07_Runtime.tex <==
\section{Algorithms' Time Complexity}
We now analyze the runtime of the algorithms introduced in this work.
\begin{lemma}
    Algorithm~\ref{alg:dp-multi-set} runs in $\tilde{O}(qf|\cal S|)$, where $q$ is the maximum set size and $f$ is the maximum frequency of any element (ignoring multiplicity).\end{lemma}
    \begin{proof}
Initially, the algorithm computes $A^{(1)}(\cdot)$ for all sets in $\cal S$, which can be done in $O(|\calS|q)$. Then the algorithm runs for $|\mathcal{S}|$ iterations, once per set, contributing the $|\mathcal{S}|$ factor. In each iteration, a set is sampled according to the exponential mechanism, where probabilities are proportional to $\exp(\varepsilon' A(S))$. Sampling can be done in $\tilde{O}(1)$.

After a set $S_j$ is selected, the algorithm updates the covering requirements for each element $e \in S_j$, which affects the utilities $A(S')$ for all other sets $S'$ containing $e$. Since each element appears in at most $f$ sets, and each set contains at most $q$ elements, the number of affected utilities per iteration is at most $qf$.
\end{proof}

As an immediate corollary of the previous lemma, we obtain the following:
\begin{theorem}
    Algorithms~\ref{alg:dp-max-deg} and~\ref{alg:explsol} each run in time $O(n\Delta^2)$, where $\Delta$ is the maximum degree of the input graph.
\end{theorem}
\begin{theorem}
    Algorithm \ref{alg:dp-walk} runs in $\tilde{O}(n\Delta^4\omega^4)$, where $\omega$ is is the matrix multiplication complexity for an $n\times n$ matrix.
\end{theorem}
\iffalse
\begin{lemma}
    Analogously to the above, Algorithm \ref{alg:dp-walk} has complexity $\tilde{O}(n\Delta^4\omega^4)$, where $\omega$ is is the matrix multiplication complexity for an $n\times n$ matrix. Each step in Line 6 removes a vertex, updating $O(\Delta^4)$ utilities. Line 10 involves counting paths of length 4, which contribute $\omega^4$. {\color{violet} The latter can likely be improved to $\tilde{O}(n\Delta^4+\omega^4)$. Count the paths once in $\omega^4$, and update the number in $O(\Delta^4)$ per iteration in Line 10. Although I am not $100\%$ sure this is correct -- depends on what data structure is used to maintain the relevant graph information.}

\end{lemma}
\fi
